The Panchromatic Hubble Andromeda Treasury: Triangulum Extended Region (PHATTER). V. The Structure of M33 in Resolved Stellar Populations

We present a detailed analysis of the the structure of the Local Group flocculent spiral galaxy M33, as measured using the Panchromatic Hubble Andromeda Treasury Triangulum Extended Region (PHATTER) survey. Leveraging the multiwavelength coverage of PHATTER, we find that the oldest populations are dominated by a smooth exponential disk with two distinct spiral arms and a classical central bar $-$ completely distinct from what is seen in broadband optical imaging, and the first-ever confirmation of a bar in M33. We estimate a bar extent of $\sim$1 kpc. The two spiral arms are asymmetric in orientation and strength, and likely represent the innermost impact of the recent tidal interaction responsible for M33's warp at larger scales. The flocculent multi-armed morphology for which M33 is known is only visible in the young upper main sequence population, which closely tracks the morphology of the ISM. We investigate the stability of M33's disk, finding $Q{\sim}1$ over the majority of the disk. We fit multiple components to the old stellar density distribution and find that, when considering recent stellar kinematics, M33's bulk structure favors the inclusion of an accreted halo component, modeled as a broken power-law. The best-fit halo model has an outer power-law index of $-$3 and accurately describes observational evidence of M33's stellar halo from both resolved stellar spectroscopy in the disk and its stellar populations at large radius. Integrating this profile yields a total halo stellar mass of ${\sim}5{\times}10^8\ M_{\odot}$, giving a total stellar halo mass fraction of 16%, most of which resides in the innermost 2.5 kpc.

==> MATCHtbl.tex <==
\newcolumntype{t}{!{\extracolsep{32pt}}l!{\extracolsep{0pt}}}
\newcolumntype{p}{!{\extracolsep{32pt}}r!{\extracolsep{0pt}}}

\begin{deluxetable}{ttp}[!t]
\tablecaption{\textnormal{MATCH Parameters for Synthetic Catalog}\label{tab:match}}
\tablecolumns{3}
\setlength{\extrarowheight}{2pt}
\tabletypesize{\small}
\tablehead{%
\colhead{Parameter} &
\colhead{Description} &
\colhead{Value} \vspace{-5mm}\\
}
%
\startdata
\texttt{IMF} & IMF Slope & 1.3 \\ 
\texttt{(m-M)$_0$} & Dist.\ modulus & 24.67 \\
\texttt{Av} & $A_V$ & 0.13 \\
\texttt{Zspread} & Metallicity spread & 0.3 \\
\texttt{BF} & Binary fraction & 0.3 \\
\texttt{dmag\_min} & Min.\ out$-$in mag & $-$0.75 \\
\enddata
\tablecomments{Parameter values used with the MATCH \texttt{fake} utility to generate the synthetic stellar catalog.}
\end{deluxetable}

==> agetbl.tex <==
\newcolumntype{t}{!{\extracolsep{28pt}}l!{\extracolsep{0pt}}}
\newcolumntype{p}{!{\extracolsep{28pt}}r!{\extracolsep{0pt}}}

\begin{deluxetable}{tppp}[t]
\tablecaption{\textnormal{Population Ages}\label{tab:ages}}
\tablecolumns{4}
\setlength{\extrarowheight}{2pt}
\tabletypesize{\small}
\tablehead{%
\colhead{} &
\colhead{50\%} &
\colhead{16\%} &
\colhead{84\%} \vspace{-2.5mm}\\
%
\colhead{Population} & 
\colhead{(Gyr)} & 
\colhead{(Gyr)} & 
\colhead{(Gyr)} \vspace{-5mm}\\ 
}
%
\startdata
MS & 0.080 & 0.022 & 0.178 \\
HeB & 0.252 & 0.141 & 0.447 \\
AGB & 1.12 & 0.56 & 2.24 \\
RGB & 3.99 & 1.42 & 8.92 \\
\enddata
\tablecomments{Median ages and 16--84\% ranges derived for synthetic stars belonging to the four different population selections.}
\end{deluxetable}
